DualRefine: Self-Supervised Depth and Pose Estimation Through Iterative Epipolar Sampling and Refinement Toward Equilibrium

Self-supervised multi-frame depth estimation achieves high accuracy by computing matching costs of pixel correspondences between adjacent frames, injecting geometric information into the network. These pixel-correspondence candidates are computed based on the relative pose estimates between the frames. Accurate pose predictions are essential for precise matching cost computation as they influence the epipolar geometry. Furthermore, improved depth estimates can, in turn, be used to align pose estimates. Inspired by traditional structure-from-motion (SfM) principles, we propose the DualRefine model, which tightly couples depth and pose estimation through a feedback loop. Our novel update pipeline uses a deep equilibrium model framework to iteratively refine depth estimates and a hidden state of feature maps by computing local matching costs based on epipolar geometry. Importantly, we used the refined depth estimates and feature maps to compute pose updates at each step. This update in the pose estimates slowly alters the epipolar geometry during the refinement process. Experimental results on the KITTI dataset demonstrate competitive depth prediction and odometry prediction performance surpassing published self-supervised baselines.

==> Figures/updates.tex <==


\begin{figure}[t!]
\begin{center}
    \begin{adjustbox}{width=0.45\textwidth}
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{c}
    \includegraphics[width=0.9\linewidth]{Figures/UpdateDepth.pdf}  \\
    (a) \\
    \\
    \hline
    \\
    \includegraphics[width=0.9\linewidth]{Figures/UpdatePose.pdf}  \\
    (b) \\
    \end{tabular}
    \end{adjustbox}
% \captionsetup{justification=centering,margin=1cm}
\caption{The recurrent alignment modules. (a) The depth updates is performed by sampling from the source feature map using the current depth and pose estimate. The sampled feature map is used to construct a cost volume which is taken as an input into the update module. (b) The pose estimates are updated in conjunction based on direct feature-metric alignments. The current depth and pose estimates are used to sample and compute the bias $b$, jacobian $\mathcal{J}$, and confidence $W$ for computing the update step.}
\label{fig:update}
\end{center}
\end{figure}

==> Tables/ablation.tex <==
\begin{table}[t]
    \begin{center}
        \begin{adjustbox}{width=0.4\textwidth}
        % \setlength{\tabcolsep}{10pt}
        \begin{tabular}{cc|ccc}
            \Xhline{4\arrayrulewidth}
            % \rowcolor{red!7}
            Pose & Consistency & \multirow{2}{*}{Abs Rel $\downarrow$} & \multirow{2}{*}{RMSE $\downarrow$} & \multirow{2}{*}{$\delta_1$ $\uparrow$} \\
            Updates & mask & & & \\
            \Xhline{4\arrayrulewidth}
            no update & $T_0$ & 0.104 & 4.656 & 0.893 \\
            no $W_{h,k}$ & $T_0$ & 0.099 & 4.375 & 0.895 \\
            all & $T_0$ & 0.093 & 4.298 & 0.903 \\
            all & $T^*$ & \textbf{0.092} & \textbf{4.285} & \textbf{0.906} \\
            \Xhline{4\arrayrulewidth}
        \end{tabular}
        \end{adjustbox}
    \caption{Ablation experiment for the effect of pose updates on the KITTI~\cite{geiger2012we} Eigen split. \textbf{Bold}: Best.}
    \vspace{-5mm}
    \label{table:ablpose}
    \end{center}
\end{table}


\begin{table}[t]
    \begin{center}
        \begin{adjustbox}{width=0.4\textwidth}
        \setlength{\tabcolsep}{8pt}
        \begin{tabular}{c|cccc}
            \Xhline{4\arrayrulewidth}
            % \rowcolor{red!7}
            DEQ & \multirow{2}{*}{Abs Rel $\downarrow$} & \multirow{2}{*}{RMSE $\downarrow$} & \multirow{2}{*}{$\delta_1$ $\uparrow$} & Time \\
            \# iters & & & & (ms) \\
            \Xhline{4\arrayrulewidth}
            3$\rightarrow$3 & 0.095 & 4.292 & 0.904 & 66 \\
            \hline
            6$\rightarrow$0 & 0.104 & 4.506 & 0.903 & 49 \\
            6$\rightarrow$3 & 0.098 & 4.424 & 0.902 & 67 \\
            6$\rightarrow$6 & \textbf{0.092} & \textbf{4.266} & 0.905 & 85 \\
            \hline
            12$\rightarrow$3 & 0.104 & 4.420 & 0.899 & 66 \\
            12$\rightarrow$6 & 0.095 & 4.337 & \textbf{0.907} & 86 \\
            12$\rightarrow$12 & \textbf{0.092} & 4.285 & 0.906 & 122\\
            
            \Xhline{4\arrayrulewidth}
        \end{tabular}
        \end{adjustbox}
    \caption{Ablation experiment for the DEQ iterations on the KITTI~\cite{geiger2012we} Eigen split. $a\rightarrow b$ represents $a :$ \# iters at training and $b :$ \# iters at test time. \textbf{Bold}: Best.}
    \vspace{-5mm}
    \label{table:abldeq}
    \end{center}
\end{table}


% \begin{table}[t]
%     \begin{center}
%         \begin{adjustbox}{width=0.4\textwidth}
%         \setlength{\tabcolsep}{8pt}
%         \begin{tabular}{c|cccc}
%             \Xhline{4\arrayrulewidth}
%             % \rowcolor{red!7}
%             DEQ & \multirow{2}{*}{Abs Rel $\downarrow$} & \multirow{2}{*}{Sq Rel $\downarrow$} & \multirow{2}{*}{RMSE $\downarrow$} & \multirow{2}{*}{$\delta_1$ $\uparrow$} \\
%             \# iters & & & \\
%             \Xhline{4\arrayrulewidth}
%             3$\rightarrow$3 & 0.095 & 0.661 & 4.292 & 0.904 \\
%             6$\rightarrow$6 & 0.092 & 0.664 & 4.266 & 0.905 \\
%             6$\rightarrow$3 & 0.098 & 0.700 & 4.424 & 0.902 \\
%             12$\rightarrow$12 & 0.092 & 0.680 & 4.280 & 0.906 \\
%             12$\rightarrow$6 & 0.095 & 0.672 & 4.337 & 0.907 \\
%             12$\rightarrow$3 & 0.104 & 0.679 & 4.420 & 0.899 \\
            
%             \Xhline{4\arrayrulewidth}
%         \end{tabular}
%         \end{adjustbox}
%     \caption{Ablation experiment for the DEQ iterations on the KITTI~\cite{geiger2012we} Eigen split. $a\rightarrow b$ represents $a :$ \# iters at training and $b :$ \# iters at test time. \textbf{Bold}: Best.}
%     \vspace{-5mm}
%     \label{table:abldeq}
%     \end{center}
% \end{table}


% \begin{table}[t]
%     % \begin{center}
%         \begin{adjustbox}{width=0.48\textwidth}
%         % \setlength{\tabcolsep}{10pt}
%         \begin{tabular}{ccc|cccc}
%             \Xhline{4\arrayrulewidth}
%             % \rowcolor{red!7}
%             Pose & \multicolumn{2}{c|}{Loss pairs} & \multirow{2}{*}{Abs Rel $\downarrow$} & \multirow{2}{*}{Sq Rel $\downarrow$} &  \multirow{2}{*}{RMSE $\downarrow$} & \multirow{2}{*}{RMSE log $\downarrow$} \\
%             Updates & $d^*$ & $T^*$ & & & & \\
%             \Xhline{4\arrayrulewidth}
%             \multicolumn{7}{c}{baseline} \\
%             \hline
%             no & $T^{[0]}$ & & 0.101 & 0.813 & 4.621 & 0.184 \\
%             \Xhline{4\arrayrulewidth}
%             \multicolumn{7}{c}{pose updates} \\
%             \hline
%             detached & $T^{[0]}$ & $d^{[0]}$ & 0.101 & 0.813 & 4.661 & 0.182 \\
%             detached & $T^{[0]}$ & $d^*$ & 0.101 & 0.798 & 4.703 & 0.184 \\
%             yes & $T^{[0]}$ & $d^{[0]}$ & 0.106 & 0.847 & 4.709 & 0.186 \\
%             yes & $T^*$ & $d^{[0]}$ & \textbf{0.098} & 0.766 & 4.574 & \textbf{0.180} \\
%             yes & $T^{[0]}$ & $d^*$ & \textbf{0.098} & \textbf{0.760} & \textbf{4.481} & \textbf{0.180} \\
%             yes & $T^*$ & $d^*$ & 0.102 & 0.859 & 4.659 & 0.185 \\
%             \Xhline{4\arrayrulewidth}
%         \end{tabular}
%         \end{adjustbox}
%     \caption{Ablation experiment for the effect of pose updates and self-supervision pairings on the KITTI~\cite{geiger2012we} Eigen split. \textbf{Bold}: Best.}
%     % \vspace{-7mm}
%     \label{table:ablation}
%     % \end{center}
% \end{table}

==> Tables/cityscapesgen.tex <==
\newcommand{\sbullets}{\tikz\draw[black,fill=black] (0,0) circle (.4ex)}

\begin{table*}[t!]
    \begin{center}
        \begin{adjustbox}{width=0.9\textwidth}
        % \setlength{\tabcolsep}{10pt}
        \begin{tabular}{c|cc|ccccccc}
            \Xhline{4\arrayrulewidth}
            % \rowcolor{red!7}
            Method & Test frames & $W\times H$ & \cellcolor{red!7} Abs Rel $\downarrow$ & \cellcolor{red!7} Sq Rel $\downarrow$ &  \cellcolor{red!7} RMSE $\downarrow$ & \cellcolor{red!7} RMSE log $\downarrow$ & \cellcolor{blue!7} $\delta_1$ $\uparrow$ & \cellcolor{blue!7} $\delta_2$ $\uparrow$ & \cellcolor{blue!7} $\delta_3$ $\uparrow$ \\
            \hline
            Monodepth2~\cite{godard2019digging} & 1 & $640\times 192$ & 0.159 & 2.016 & 8.074 & 0.221 & 0.787 & 0.941 & 0.978 \\
            ManyDepth~\cite{watson2021temporal} & 2 (-1, 0) & $640\times 192$ & 0.137 & 1.578 & 7.249 & 0.197 & 0.827 & 0.954 & 0.985 \\
            \cellcolor{green!7}
            DualRefine (initial) & 2 (-1, 0) & $640\times 192$ & 0.142 & 1.545 & 7.946 & 0.210 & 0.811 & 0.944 & 0.983 \\
            \cellcolor{green!7}
            DualRefine (refined) & 2 (-1, 0) & $640\times 192$ & \underbar{0.058} & \underbar{0.294} & \underbar{3.062} & \underbar{0.097} & \textbf{0.956} & \textbf{0.992} & \textbf{0.998} \\
            \Xhline{4\arrayrulewidth}
        \end{tabular}
        \end{adjustbox}
    \caption{Results and comparison with other state-of-the-arts models on the KITTI~\cite{geiger2012we} Eigen split~\cite{eigen2014depth} with improved depth maps~\cite{uhrig2017sparsity}. \textbf{Bold}: Best, \underbar{Underscore}: Second best. $^\dagger:$ evaluated on whole sequences}
    \vspace{-5mm}
    \label{table:improved}
    \end{center}
\end{table*}

